How Does Sharpness-Aware Minimization Minimize Sharpness?

Sharpness-Aware Minimization (SAM) is a highly effective regularization technique for improving the generalization of deep neural networks for various settings. However, the underlying working of SAM remains elusive because of various intriguing approximations in the theoretical characterizations. SAM intends to penalize a notion of sharpness of the model but implements a computationally efficient variant; moreover, a third notion of sharpness was used for proving generalization guarantees. The subtle differences in these notions of sharpness can indeed lead to significantly different empirical results. This paper rigorously nails down the exact sharpness notion that SAM regularizes and clarifies the underlying mechanism. We also show that the two steps of approximations in the original motivation of SAM individually lead to inaccurate local conclusions, but their combination accidentally reveals the correct effect, when full-batch gradients are applied. Furthermore, we also prove that the stochastic version of SAM in fact regularizes the third notion of sharpness mentioned above, which is most likely to be the preferred notion for practical performance. The key mechanism behind this intriguing phenomenon is the alignment between the gradient and the top eigenvector of Hessian when SAM is applied.

==> intro_old.tex <==
\section{Introduction}\label{sec:intro}



Modern deep nets are often overparametrized and have the capacity to  fit even randomly labeled data~\citep{zhang2016understanding}. Thus, a small training loss does not necessarily imply good generalization.
Yet, standard gradient-based training algorithms such as SGD are able to find generalizable models.
Recent empirical and theoretical studies suggest that generalization is well-correlated with the sharpness of the loss landscape around the learned parameter~\cite{keskar2016large,dinh2017sharp,dziugaite2017computing,neyshabur2017exploring,jiang2019fantastic}. %
Partly motivated by these studies, \cite{foret2021sharpnessaware,wu2020adversarial,zheng2021regularizing} propose to penalize the sharpness of the landscape along the worst-case direction. %
We refer this method to \emph{Sharpness-Aware Minimization}~(SAM) and focus on the  version of \citet{foret2021sharpnessaware} in this paper.
More specifically, SAM aims to solve the following optimization problem:
\begin{align}\label{eq:max_sharpness}
\min_{x}  \maxloss(x),\quad  \textrm{where}\quad \maxloss(x)	= \max_{\norm{v}_2\le 1} L(x+\rho v),
\end{align}
where $L$ is the training loss, $x$ is the parameter and $\rho$ is the \emph{perturbation radius}, a hyperparameter requiring tuning. Throughout this paper, we call $\maxsharpness(x) =\maxloss(x)-L(x)$ the \emph{worst-direction sharpness} at $x$ and thus SAM is minimizing the original training loss plus the worst-direction sharpness at x.

However, even evaluation of $\maxloss(x)$ is computationally expansive, not to mention optimization. Thus \cite{foret2021sharpnessaware,zheng2021regularizing} proposed to approximate the direction $v$ in the worst-direction sharpness by the direction of gradient ascent on $L(x)$, which yields the following surrogate optimization problem. We call $\ascsharpness(x)=\ascloss(x)-L(x)$ the \emph{ascent-direction sharpness} at $x$.
\begin{align}\label{eq:asc_sharpness}
\min_{x}  \ascloss(x),\quad  \textrm{where}\quad \ascloss(x)	= L\left(x+\rho \frac{\nabla L(x)}{\norm{\nabla L(x)}_2}\right).
\end{align}



For further acceleration, \citet{foret2021sharpnessaware,zheng2021regularizing} omits the gradient through other occurrence of $x$ and approximate the gradient of ascent-direction sharpness by gradient taken after one-step ascent, \emph{i.e.}, $\nabla \ascloss(x) \approx \nabla L\left(x+\rho \frac{\nabla L(x)}{\norm{\nabla L(x)}_2}\right)$ and derive the update rule of SAM, where $\eta$ is the learning rate. 
\begin{align}\label{eq:sam}
\textrm{Sharpness-Aware Minimization (SAM):} \quad x(t+1) = x(t) -\eta  \nabla L\left(x+\rho \frac{\nabla L(x)}{\norm{\nabla L(x)}_2}\right) \qquad
\end{align}

The empirical success of SAM is not possible without these two approximations for computational efficiency--- (1) approximating $\maxloss$ by $\ascloss$ and (2) approximating  $\nabla \ascloss(x)$ by $\nabla L\left(x+\rho \frac{\nabla L(x)}{\norm{\nabla L(x)}_2}\right)$. Yet they also limit our theoretical understanding of the mechanism behind the success, as both approximations are heuristic and lack of rigorous mathematical explanations. It is not theoretically clear whether SAM indeed solves the optimization problem~\eqref{eq:max_sharpness}.  

Besides optimization, there are also mismatches on the generalization side. First, the existing generalization theory for SAM~\citep{foret2021sharpnessaware,wu2020adversarial} upper bounds the worst-direction sharpness by the average-direction sharpness (see ??) and then invoke the PAC Bayesian theory~\citep{mcallester2003simplified}. Intriguingly, minimizing average-direction sharpness by random perturbation doesn't lead to competitive generalization as SAM does~\citep{foret2021sharpnessaware,wu2020adversarial}. Second, in practice people typically run SAM on a stochastic loss, where the loss $L$ is replaced by the mini-batch loss in the update rule \eqref{eq:sam}. Empirically it is observed that the generalization of SAM improves as the batch size decreases and thus \citet{foret2021sharpnessaware} argued that the stochastic worst-case sharpness, \emph{i.e.},  the expected worst-direction sharpness of the stochastic loss~\cite{foret2021sharpnessaware}, is a  regularizer with better generalization as the sharpness decreases. However,  current theory not only cannot distinguish the sharpness with the different batch sizes, but also cannot guarantee that SAM does minimize the stochastic worst-case sharpness.




In this paper, we answer the above questions by solving the explicit bias of various notions of sharpness and analyzing the optimization trajectory of SAM. Our analysis is performed for small perturbation radius $\rho$ and learning rate and under the setting where the minimizers of loss form a manifold following ~\citep{fehrman2020convergence,li2021happens}  In particular, we make the following contributions.

\begin{enumerate}
	\item In the full-batch setting, we prove that SAM does minimize worst-direction sharpness locally . But surprisingly, this is not due to the \emph{explicit bias} of minimizing ascent-direction sharpness, but the \emph{implicit bias} of the specific approximation made by SAM. 

	\item Indeed both heuristic approximations mentioned above lead to inaccurate solutions, that is, (1) minimizing worst-direction sharpness and ascent-direction sharpness induce different biases among minimizers and (2) SAM doesn't minimize ascent-direction sharpness.  

		In detail, we show regularizing worst- (or ascent-direction) sharpness have the same effect of regularizing the top (or smallest non-zero) eigenvalue of the Hessian of the original loss.
		
	\item We extend our analysis to the stochastic case where the batch size is $1$.  Under this setting we show minimizing stochastic worst-, ascent- and average-direction sharpness has the same bias of preferring minimizers with small trace of Hessian. We also show that SAM implicitly minimizes the trace of Hessian. (\Cref{1sam})
		
	\item	As implications, our theory explains how SAM can have a different implicit bias in the stochastic setting. This explanation is consistent with the existing generalization bound~\citep{foret2021sharpnessaware} which essentially uses average-direction sharpness as a generalization measure. Moreover, despite minimizing average-direction sharpness by SGD also has the explicit bias of finding minimizers with a small trace of Hessian, our theorem ?? shows that its regularization strength is $D$ times weaker than stochastic SAM provided the same perturbation radius $\rho$, where $D$ is the number of parameters which is typically larger than a million. This might be accountable for the empirical failure of average-direction sharpness as an explicit regularizer as the regularization effect is too weak. On the other hand, a much larger perturbation radius can make optimization difficult.
\end{enumerate}


\begin{table}[h!]
\centering
 \begin{tabular}{c| c c c} 

 Type of Sharpness & Symbol & Definition & Explicit Bias Among Minimizers \\ 
 \hline
 Worst-direction  & $\maxloss$ & $\max_{\norm{v}_2\le 1} L(x+\rho v)$ & $\min_x \lambda_1(\nabla^ 2L(x))$ \\ 
 Ascent-direction  & $\ascloss$ & $L\left(x+\rho \frac{\nabla L(x)}{\norm{\nabla L(x)}_2}\right)$ & $\min_x \lambda_{\textrm{min}}(\nabla^ 2L(x))$ \\ 
  Average-direction  & $\avgloss$ & $\E_{v\sim N(0,I)} L(x+\rho \frac{v}{\norm{v}_2})$ & $\min_x \mathrm{Tr}(\nabla^ 2L(x))$  
 \end{tabular}
 \caption{Definitions and explicit biases of different notions of sharpness. Here $\lambda_{\textrm{min}}$ denotes to the smallest \emph{non-zero} eigenvalue.}\label{tb:main}
\end{table}


